Measurements of Sigma+ and Sigma- Time-like Electromagnetic Form Factors for center-of-mass energies from 2.3864 to 3.0200 GeV

The Born cross sections of the $e^{+}e^{-}\to\Sigma^{+}\bar{\Sigma}^{-}$ and $e^{+}e^{-}\to\Sigma^{-}\bar{\Sigma}^{+}$ processes are determined with high precision for center-of-mass energy from 2.3864 to 3.0200 GeV with the BESIII detector. Nonzero cross sections near threshold are observed. The resulting ratio of effective form factors for the $\Sigma^{+}$ and $\Sigma^{-}$ is consistent with 3, agreeing with the ratio of the incoherent sum of the squared charges of the $\Sigma^{+}$ and $\Sigma^{-}$ valence quarks, but disagreeing with various theoretical predictions. In addition, ratios of the $\Sigma^{+}$ electric and magnetic form factors, $|G_{E}/G_{M}|$, are obtained at three center-of-mass energies through an analysis of the angular distributions. These measurements, which are studied for the first time in the off-resonance region, provide precision experimental input for understanding baryonic structure. The observed novel features of the $\Sigma^{\pm}$ form factors require a new theoretical description for the hyperons.

==> author.tex <==
\author{
  \begin{small}
    \begin{center}
M.~Ablikim$^{1}$, M.~N.~Achasov$^{10,c}$, P.~Adlarson$^{64}$, S. ~Ahmed$^{15}$, M.~Albrecht$^{4}$, R.~Aliberti$^{28}$, A.~Amoroso$^{63A,63C}$, Q.~An$^{60,48}$, ~Anita$^{21}$, X.~H.~Bai$^{54}$, Y.~Bai$^{47}$, O.~Bakina$^{29}$, R.~Baldini Ferroli$^{23A}$, I.~Balossino$^{24A}$, Y.~Ban$^{38,k}$, K.~Begzsuren$^{26}$, J.~V.~Bennett$^{5}$, N.~Berger$^{28}$, M.~Bertani$^{23A}$, D.~Bettoni$^{24A}$, F.~Bianchi$^{63A,63C}$, J~Biernat$^{64}$, J.~Bloms$^{57}$, A.~Bortone$^{63A,63C}$, I.~Boyko$^{29}$, R.~A.~Briere$^{5}$, H.~Cai$^{65}$, X.~Cai$^{1,48}$, A.~Calcaterra$^{23A}$, G.~F.~Cao$^{1,52}$, N.~Cao$^{1,52}$, S.~A.~Cetin$^{51B}$, J.~F.~Chang$^{1,48}$, W.~L.~Chang$^{1,52}$, G.~Chelkov$^{29,b}$, D.~Y.~Chen$^{6}$, G.~Chen$^{1}$, H.~S.~Chen$^{1,52}$, M.~L.~Chen$^{1,48}$, S.~J.~Chen$^{36}$, X.~R.~Chen$^{25}$, Y.~B.~Chen$^{1,48}$, Z.~J~Chen$^{20,l}$, W.~S.~Cheng$^{63C}$, G.~Cibinetto$^{24A}$, F.~Cossio$^{63C}$, X.~F.~Cui$^{37}$, H.~L.~Dai$^{1,48}$, J.~P.~Dai$^{42,g}$, X.~C.~Dai$^{1,52}$, A.~Dbeyssi$^{15}$, R.~ B.~de Boer$^{4}$, D.~Dedovich$^{29}$, Z.~Y.~Deng$^{1}$, A.~Denig$^{28}$, I.~Denysenko$^{29}$, M.~Destefanis$^{63A,63C}$, F.~De~Mori$^{63A,63C}$, Y.~Ding$^{34}$, C.~Dong$^{37}$, J.~Dong$^{1,48}$, L.~Y.~Dong$^{1,52}$, M.~Y.~Dong$^{1,48,52}$, S.~X.~Du$^{68}$, J.~Fang$^{1,48}$, S.~S.~Fang$^{1,52}$, Y.~Fang$^{1}$, R.~Farinelli$^{24A}$, L.~Fava$^{63B,63C}$, F.~Feldbauer$^{4}$, G.~Felici$^{23A}$, C.~Q.~Feng$^{60,48}$, M.~Fritsch$^{4}$, C.~D.~Fu$^{1}$, Y.~Fu$^{1}$, X.~L.~Gao$^{60,48}$, Y.~Gao$^{61}$, Y.~Gao$^{38,k}$, Y.~G.~Gao$^{6}$, I.~Garzia$^{24A,24B}$, E.~M.~Gersabeck$^{55}$, A.~Gilman$^{56}$, K.~Goetzen$^{11}$, L.~Gong$^{37}$, W.~X.~Gong$^{1,48}$, W.~Gradl$^{28}$, M.~Greco$^{63A,63C}$, L.~M.~Gu$^{36}$, M.~H.~Gu$^{1,48}$, S.~Gu$^{2}$, Y.~T.~Gu$^{13}$, C.~Y~Guan$^{1,52}$, A.~Q.~Guo$^{22}$, L.~B.~Guo$^{35}$, R.~P.~Guo$^{40}$, Y.~P.~Guo$^{28}$, Y.~P.~Guo$^{9,h}$, A.~Guskov$^{29}$, S.~Han$^{65}$, T.~T.~Han$^{41}$, T.~Z.~Han$^{9,h}$, X.~Q.~Hao$^{16}$, F.~A.~Harris$^{53}$, K.~L.~He$^{1,52}$, F.~H.~Heinsius$^{4}$, C.~H.~Heinz$^{28}$, T.~Held$^{4}$, Y.~K.~Heng$^{1,48,52}$, M.~Himmelreich$^{11,f}$, T.~Holtmann$^{4}$, Y.~R.~Hou$^{52}$, Z.~L.~Hou$^{1}$, H.~M.~Hu$^{1,52}$, J.~F.~Hu$^{42,g}$, T.~Hu$^{1,48,52}$, Y.~Hu$^{1}$, G.~S.~Huang$^{60,48}$, L.~Q.~Huang$^{61}$, X.~T.~Huang$^{41}$, Y.~P.~Huang$^{1}$, Z.~Huang$^{38,k}$, N.~Huesken$^{57}$, T.~Hussain$^{62}$, W.~Ikegami Andersson$^{64}$, W.~Imoehl$^{22}$, M.~Irshad$^{60,48}$, S.~Jaeger$^{4}$, S.~Janchiv$^{26,j}$, Q.~Ji$^{1}$, Q.~P.~Ji$^{16}$, X.~B.~Ji$^{1,52}$, X.~L.~Ji$^{1,48}$, H.~B.~Jiang$^{41}$, X.~S.~Jiang$^{1,48,52}$, X.~Y.~Jiang$^{37}$, J.~B.~Jiao$^{41}$, Z.~Jiao$^{18}$, S.~Jin$^{36}$, Y.~Jin$^{54}$, T.~Johansson$^{64}$, N.~Kalantar-Nayestanaki$^{31}$, X.~S.~Kang$^{34}$, R.~Kappert$^{31}$, M.~Kavatsyuk$^{31}$, B.~C.~Ke$^{43,1}$, I.~K.~Keshk$^{4}$, A.~Khoukaz$^{57}$, P. ~Kiese$^{28}$, R.~Kiuchi$^{1}$, R.~Kliemt$^{11}$, L.~Koch$^{30}$, O.~B.~Kolcu$^{51B,e}$, B.~Kopf$^{4}$, M.~Kuemmel$^{4}$, M.~Kuessner$^{4}$, A.~Kupsc$^{64}$, M.~ G.~Kurth$^{1,52}$, W.~K\"uhn$^{30}$, J.~J.~Lane$^{55}$, J.~S.~Lange$^{30}$, P. ~Larin$^{15}$, L.~Lavezzi$^{63C}$, H.~Leithoff$^{28}$, M.~Lellmann$^{28}$, T.~Lenz$^{28}$, C.~Li$^{39}$, C.~H.~Li$^{33}$, Cheng~Li$^{60,48}$, D.~M.~Li$^{68}$, F.~Li$^{1,48}$, G.~Li$^{1}$, H.~Li$^{43}$, H.~B.~Li$^{1,52}$, H.~J.~Li$^{9,h}$, J.~L.~Li$^{41}$, J.~Q.~Li$^{4}$, Ke~Li$^{1}$, L.~K.~Li$^{1}$, Lei~Li$^{3}$, P.~L.~Li$^{60,48}$, P.~R.~Li$^{32}$, S.~Y.~Li$^{50}$, W.~D.~Li$^{1,52}$, W.~G.~Li$^{1}$, X.~H.~Li$^{60,48}$, X.~L.~Li$^{41}$, Z.~B.~Li$^{49}$, Z.~Y.~Li$^{49}$, H.~Liang$^{1,52}$, H.~Liang$^{60,48}$, Y.~F.~Liang$^{45}$, Y.~T.~Liang$^{25}$, L.~Z.~Liao$^{1,52}$, J.~Libby$^{21}$, C.~X.~Lin$^{49}$, B.~Liu$^{42,g}$, B.~J.~Liu$^{1}$, C.~X.~Liu$^{1}$, D.~Liu$^{60,48}$, D.~Y.~Liu$^{42,g}$, F.~H.~Liu$^{44}$, Fang~Liu$^{1}$, Feng~Liu$^{6}$, H.~B.~Liu$^{13}$, H.~M.~Liu$^{1,52}$, Huanhuan~Liu$^{1}$, Huihui~Liu$^{17}$, J.~B.~Liu$^{60,48}$, J.~Y.~Liu$^{1,52}$, K.~Liu$^{1}$, K.~Y.~Liu$^{34}$, Ke~Liu$^{6}$, L.~Liu$^{60,48}$, Q.~Liu$^{52}$, S.~B.~Liu$^{60,48}$, Shuai~Liu$^{46}$, T.~Liu$^{1,52}$, X.~Liu$^{32}$, Y.~B.~Liu$^{37}$, Z.~A.~Liu$^{1,48,52}$, Z.~Q.~Liu$^{41}$, Y. ~F.~Long$^{38,k}$, X.~C.~Lou$^{1,48,52}$, F.~X.~Lu$^{16}$, H.~J.~Lu$^{18}$, J.~D.~Lu$^{1,52}$, J.~G.~Lu$^{1,48}$, X.~L.~Lu$^{1}$, Y.~Lu$^{1}$, Y.~P.~Lu$^{1,48}$, C.~L.~Luo$^{35}$, M.~X.~Luo$^{67}$, P.~W.~Luo$^{49}$, T.~Luo$^{9,h}$, X.~L.~Luo$^{1,48}$, S.~Lusso$^{63C}$, X.~R.~Lyu$^{52}$, F.~C.~Ma$^{34}$, H.~L.~Ma$^{1}$, L.~L. ~Ma$^{41}$, M.~M.~Ma$^{1,52}$, Q.~M.~Ma$^{1}$, R.~Q.~Ma$^{1,52}$, R.~T.~Ma$^{52}$, X.~N.~Ma$^{37}$, X.~X.~Ma$^{1,52}$, X.~Y.~Ma$^{1,48}$, Y.~M.~Ma$^{41}$, F.~E.~Maas$^{15}$, M.~Maggiora$^{63A,63C}$, S.~Maldaner$^{28}$, S.~Malde$^{58}$, Q.~A.~Malik$^{62}$, A.~Mangoni$^{23B}$, Y.~J.~Mao$^{38,k}$, Z.~P.~Mao$^{1}$, S.~Marcello$^{63A,63C}$, Z.~X.~Meng$^{54}$, J.~G.~Messchendorp$^{31}$, G.~Mezzadri$^{24A}$, T.~J.~Min$^{36}$, R.~E.~Mitchell$^{22}$, X.~H.~Mo$^{1,48,52}$, Y.~J.~Mo$^{6}$, N.~Yu.~Muchnoi$^{10,c}$, H.~Muramatsu$^{56}$, S.~Nakhoul$^{11,f}$, Y.~Nefedov$^{29}$, F.~Nerling$^{11,f}$, I.~B.~Nikolaev$^{10,c}$, Z.~Ning$^{1,48}$, S.~Nisar$^{8,i}$, S.~L.~Olsen$^{52}$, Q.~Ouyang$^{1,48,52}$, S.~Pacetti$^{23B,23C}$, X.~Pan$^{9,h}$, Y.~Pan$^{55}$, A.~Pathak$^{1}$, P.~Patteri$^{23A}$, M.~Pelizaeus$^{4}$, H.~P.~Peng$^{60,48}$, K.~Peters$^{11,f}$, J.~Pettersson$^{64}$, J.~L.~Ping$^{35}$, R.~G.~Ping$^{1,52}$, A.~Pitka$^{4}$, R.~Poling$^{56}$, V.~Prasad$^{60,48}$, H.~Qi$^{60,48}$, H.~R.~Qi$^{50}$, M.~Qi$^{36}$, T.~Y.~Qi$^{9}$, T.~Y.~Qi$^{2}$, S.~Qian$^{1,48}$, W.-B.~Qian$^{52}$, Z.~Qian$^{49}$, C.~F.~Qiao$^{52}$, L.~Q.~Qin$^{12}$, X.~S.~Qin$^{4}$, Z.~H.~Qin$^{1,48}$, J.~F.~Qiu$^{1}$, S.~Q.~Qu$^{37}$, K.~H.~Rashid$^{62}$, K.~Ravindran$^{21}$, C.~F.~Redmer$^{28}$, A.~Rivetti$^{63C}$, V.~Rodin$^{31}$, M.~Rolo$^{63C}$, G.~Rong$^{1,52}$, Ch.~Rosner$^{15}$, M.~Rump$^{57}$, A.~Sarantsev$^{29,d}$, Y.~Schelhaas$^{28}$, C.~Schnier$^{4}$, K.~Schoenning$^{64}$, M.~Scodeggio$^{24A}$, D.~C.~Shan$^{46}$, W.~Shan$^{19}$, X.~Y.~Shan$^{60,48}$, M.~Shao$^{60,48}$, C.~P.~Shen$^{9}$, P.~X.~Shen$^{37}$, X.~Y.~Shen$^{1,52}$, H.~C.~Shi$^{60,48}$, R.~S.~Shi$^{1,52}$, X.~Shi$^{1,48}$, X.~D~Shi$^{60,48}$, J.~J.~Song$^{41}$, Q.~Q.~Song$^{60,48}$, W.~M.~Song$^{27,1}$, Y.~X.~Song$^{38,k}$, S.~Sosio$^{63A,63C}$, S.~Spataro$^{63A,63C}$, F.~F. ~Sui$^{41}$, G.~X.~Sun$^{1}$, J.~F.~Sun$^{16}$, L.~Sun$^{65}$, S.~S.~Sun$^{1,52}$, T.~Sun$^{1,52}$, W.~Y.~Sun$^{35}$, X~Sun$^{20,l}$, Y.~J.~Sun$^{60,48}$, Y.~K.~Sun$^{60,48}$, Y.~Z.~Sun$^{1}$, Z.~T.~Sun$^{1}$, Y.~H.~Tan$^{65}$, Y.~X.~Tan$^{60,48}$, C.~J.~Tang$^{45}$, G.~Y.~Tang$^{1}$, J.~Tang$^{49}$, V.~Thoren$^{64}$, B.~Tsednee$^{26}$, I.~Uman$^{51D}$, B.~Wang$^{1}$, B.~L.~Wang$^{52}$, C.~W.~Wang$^{36}$, D.~Y.~Wang$^{38,k}$, H.~P.~Wang$^{1,52}$, K.~Wang$^{1,48}$, L.~L.~Wang$^{1}$, M.~Wang$^{41}$, M.~Z.~Wang$^{38,k}$, Meng~Wang$^{1,52}$, W.~H.~Wang$^{65}$, W.~P.~Wang$^{60,48}$, X.~Wang$^{38,k}$, X.~F.~Wang$^{32}$, X.~L.~Wang$^{9,h}$, Y.~Wang$^{60,48}$, Y.~Wang$^{49}$, Y.~D.~Wang$^{15}$, Y.~F.~Wang$^{1,48,52}$, Y.~Q.~Wang$^{1}$, Z.~Wang$^{1,48}$, Z.~Y.~Wang$^{1}$, Ziyi~Wang$^{52}$, Zongyuan~Wang$^{1,52}$, D.~H.~Wei$^{12}$, P.~Weidenkaff$^{28}$, F.~Weidner$^{57}$, S.~P.~Wen$^{1}$, D.~J.~White$^{55}$, U.~Wiedner$^{4}$, G.~Wilkinson$^{58}$, M.~Wolke$^{64}$, L.~Wollenberg$^{4}$, J.~F.~Wu$^{1,52}$, L.~H.~Wu$^{1}$, L.~J.~Wu$^{1,52}$, X.~Wu$^{9,h}$, Z.~Wu$^{1,48}$, L.~Xia$^{60,48}$, H.~Xiao$^{9,h}$, S.~Y.~Xiao$^{1}$, Y.~J.~Xiao$^{1,52}$, Z.~J.~Xiao$^{35}$, X.~H.~Xie$^{38,k}$, Y.~G.~Xie$^{1,48}$, Y.~H.~Xie$^{6}$, T.~Y.~Xing$^{1,52}$, X.~A.~Xiong$^{1,52}$, G.~F.~Xu$^{1}$, J.~J.~Xu$^{36}$, Q.~J.~Xu$^{14}$, W.~Xu$^{1,52}$, X.~P.~Xu$^{46}$, F.~Yan$^{9,h}$, L.~Yan$^{9,h}$, L.~Yan$^{63A,63C}$, W.~B.~Yan$^{60,48}$, W.~C.~Yan$^{68}$, Xu~Yan$^{46}$, H.~J.~Yang$^{42,g}$, H.~X.~Yang$^{1}$, L.~Yang$^{65}$, R.~X.~Yang$^{60,48}$, S.~L.~Yang$^{1,52}$, Y.~H.~Yang$^{36}$, Y.~X.~Yang$^{12}$, Yifan~Yang$^{1,52}$, Zhi~Yang$^{25}$, M.~Ye$^{1,48}$, M.~H.~Ye$^{7}$, J.~H.~Yin$^{1}$, Z.~Y.~You$^{49}$, B.~X.~Yu$^{1,48,52}$, C.~X.~Yu$^{37}$, G.~Yu$^{1,52}$, J.~S.~Yu$^{20,l}$, T.~Yu$^{61}$, C.~Z.~Yuan$^{1,52}$, W.~Yuan$^{63A,63C}$, X.~Q.~Yuan$^{38,k}$, Y.~Yuan$^{1}$, Z.~Y.~Yuan$^{49}$, C.~X.~Yue$^{33}$, A.~Yuncu$^{51B,a}$, A.~A.~Zafar$^{62}$, Y.~Zeng$^{20,l}$, B.~X.~Zhang$^{1}$, Guangyi~Zhang$^{16}$, H.~H.~Zhang$^{49}$, H.~Y.~Zhang$^{1,48}$, J.~L.~Zhang$^{66}$, J.~Q.~Zhang$^{4}$, J.~W.~Zhang$^{1,48,52}$, J.~Y.~Zhang$^{1}$, J.~Z.~Zhang$^{1,52}$, Jianyu~Zhang$^{1,52}$, Jiawei~Zhang$^{1,52}$, L.~Zhang$^{1}$, Lei~Zhang$^{36}$, S.~Zhang$^{49}$, S.~F.~Zhang$^{36}$, T.~J.~Zhang$^{42,g}$, X.~Y.~Zhang$^{41}$, Y.~Zhang$^{58}$, Y.~H.~Zhang$^{1,48}$, Y.~T.~Zhang$^{60,48}$, Yan~Zhang$^{60,48}$, Yao~Zhang$^{1}$, Yi~Zhang$^{9,h}$, Z.~H.~Zhang$^{6}$, Z.~Y.~Zhang$^{65}$, G.~Zhao$^{1}$, J.~Zhao$^{33}$, J.~Y.~Zhao$^{1,52}$, J.~Z.~Zhao$^{1,48}$, Lei~Zhao$^{60,48}$, Ling~Zhao$^{1}$, M.~G.~Zhao$^{37}$, Q.~Zhao$^{1}$, S.~J.~Zhao$^{68}$, Y.~B.~Zhao$^{1,48}$, Y.~X.~Zhao$^{25}$, Z.~G.~Zhao$^{60,48}$, A.~Zhemchugov$^{29,b}$, B.~Zheng$^{61}$, J.~P.~Zheng$^{1,48}$, Y.~Zheng$^{38,k}$, Y.~H.~Zheng$^{52}$, B.~Zhong$^{35}$, C.~Zhong$^{61}$, L.~P.~Zhou$^{1,52}$, Q.~Zhou$^{1,52}$, X.~Zhou$^{65}$, X.~K.~Zhou$^{52}$, X.~R.~Zhou$^{60,48}$, A.~N.~Zhu$^{1,52}$, J.~Zhu$^{37}$, K.~Zhu$^{1}$, K.~J.~Zhu$^{1,48,52}$, S.~H.~Zhu$^{59}$, W.~J.~Zhu$^{37}$, X.~L.~Zhu$^{50}$, Y.~C.~Zhu$^{60,48}$, Z.~A.~Zhu$^{1,52}$, B.~S.~Zou$^{1}$, J.~H.~Zou$^{1}$
\\
\vspace{0.2cm}
(BESIII Collaboration)\\
\vspace{0.2cm} {\it
$^{1}$ Institute of High Energy Physics, Beijing 100049, People's Republic of China\\
$^{2}$ Beihang University, Beijing 100191, People's Republic of China\\
$^{3}$ Beijing Institute of Petrochemical Technology, Beijing 102617, People's Republic of China\\
$^{4}$ Bochum Ruhr-University, D-44780 Bochum, Germany\\
$^{5}$ Carnegie Mellon University, Pittsburgh, Pennsylvania 15213, USA\\
$^{6}$ Central China Normal University, Wuhan 430079, People's Republic of China\\
$^{7}$ China Center of Advanced Science and Technology, Beijing 100190, People's Republic of China\\
$^{8}$ COMSATS University Islamabad, Lahore Campus, Defence Road, Off Raiwind Road, 54000 Lahore, Pakistan\\
$^{9}$ Fudan University, Shanghai 200443, People's Republic of China\\
$^{10}$ G.I. Budker Institute of Nuclear Physics SB RAS (BINP), Novosibirsk 630090, Russia\\
$^{11}$ GSI Helmholtzcentre for Heavy Ion Research GmbH, D-64291 Darmstadt, Germany\\
$^{12}$ Guangxi Normal University, Guilin 541004, People's Republic of China\\
$^{13}$ Guangxi University, Nanning 530004, People's Republic of China\\
$^{14}$ Hangzhou Normal University, Hangzhou 310036, People's Republic of China\\
$^{15}$ Helmholtz Institute Mainz, Johann-Joachim-Becher-Weg 45, D-55099 Mainz, Germany\\
$^{16}$ Henan Normal University, Xinxiang 453007, People's Republic of China\\
$^{17}$ Henan University of Science and Technology, Luoyang 471003, People's Republic of China\\
$^{18}$ Huangshan College, Huangshan 245000, People's Republic of China\\
$^{19}$ Hunan Normal University, Changsha 410081, People's Republic of China\\
$^{20}$ Hunan University, Changsha 410082, People's Republic of China\\
$^{21}$ Indian Institute of Technology Madras, Chennai 600036, India\\
$^{22}$ Indiana University, Bloomington, Indiana 47405, USA\\
$^{23}$ (A)INFN Laboratori Nazionali di Frascati, I-00044, Frascati, Italy; (B)INFN Sezione di Perugia, I-06100, Perugia, Italy; (C)University of Perugia, I-06100, Perugia, Italy\\
$^{24}$ (A)INFN Sezione di Ferrara, I-44122, Ferrara, Italy; (B)University of Ferrara, I-44122, Ferrara, Italy\\
$^{25}$ Institute of Modern Physics, Lanzhou 730000, People's Republic of China\\
$^{26}$ Institute of Physics and Technology, Peace Ave. 54B, Ulaanbaatar 13330, Mongolia\\
$^{27}$ Jilin University, Changchun 130012, People's Republic of China\\
$^{28}$ Johannes Gutenberg University of Mainz, Johann-Joachim-Becher-Weg 45, D-55099 Mainz, Germany\\
$^{29}$ Joint Institute for Nuclear Research, 141980 Dubna, Moscow region, Russia\\
$^{30}$ Justus-Liebig-Universitaet Giessen, II. Physikalisches Institut, Heinrich-Buff-Ring 16, D-35392 Giessen, Germany\\
$^{31}$ KVI-CART, University of Groningen, NL-9747 AA Groningen, The Netherlands\\
$^{32}$ Lanzhou University, Lanzhou 730000, People's Republic of China\\
$^{33}$ Liaoning Normal University, Dalian 116029, People's Republic of China\\
$^{34}$ Liaoning University, Shenyang 110036, People's Republic of China\\
$^{35}$ Nanjing Normal University, Nanjing 210023, People's Republic of China\\
$^{36}$ Nanjing University, Nanjing 210093, People's Republic of China\\
$^{37}$ Nankai University, Tianjin 300071, People's Republic of China\\
$^{38}$ Peking University, Beijing 100871, People's Republic of China\\
$^{39}$ Qufu Normal University, Qufu 273165, People's Republic of China\\
$^{40}$ Shandong Normal University, Jinan 250014, People's Republic of China\\
$^{41}$ Shandong University, Jinan 250100, People's Republic of China\\
$^{42}$ Shanghai Jiao Tong University, Shanghai 200240, People's Republic of China\\
$^{43}$ Shanxi Normal University, Linfen 041004, People's Republic of China\\
$^{44}$ Shanxi University, Taiyuan 030006, People's Republic of China\\
$^{45}$ Sichuan University, Chengdu 610064, People's Republic of China\\
$^{46}$ Soochow University, Suzhou 215006, People's Republic of China\\
$^{47}$ Southeast University, Nanjing 211100, People's Republic of China\\
$^{48}$ State Key Laboratory of Particle Detection and Electronics, Beijing 100049, Hefei 230026, People's Republic of China\\
$^{49}$ Sun Yat-Sen University, Guangzhou 510275, People's Republic of China\\
$^{50}$ Tsinghua University, Beijing 100084, People's Republic of China\\
$^{51}$ (A)Ankara University, 06100 Tandogan, Ankara, Turkey; (B)Istanbul Bilgi University, 34060 Eyup, Istanbul, Turkey; (C)Uludag University, 16059 Bursa, Turkey; (D)Near East University, Nicosia, North Cyprus, Mersin 10, Turkey\\
$^{52}$ University of Chinese Academy of Sciences, Beijing 100049, People's Republic of China\\
$^{53}$ University of Hawaii, Honolulu, Hawaii 96822, USA\\
$^{54}$ University of Jinan, Jinan 250022, People's Republic of China\\
$^{55}$ University of Manchester, Oxford Road, Manchester, M13 9PL, United Kingdom\\
$^{56}$ University of Minnesota, Minneapolis, Minnesota 55455, USA\\
$^{57}$ University of Muenster, Wilhelm-Klemm-Str. 9, 48149 Muenster, Germany\\
$^{58}$ University of Oxford, Keble Rd, Oxford, UK OX13RH\\
$^{59}$ University of Science and Technology Liaoning, Anshan 114051, People's Republic of China\\
$^{60}$ University of Science and Technology of China, Hefei 230026, People's Republic of China\\
$^{61}$ University of South China, Hengyang 421001, People's Republic of China\\
$^{62}$ University of the Punjab, Lahore-54590, Pakistan\\
$^{63}$ (A)University of Turin, I-10125, Turin, Italy; (B)University of Eastern Piedmont, I-15121, Alessandria, Italy; (C)INFN, I-10125, Turin, Italy\\
$^{64}$ Uppsala University, Box 516, SE-75120 Uppsala, Sweden\\
$^{65}$ Wuhan University, Wuhan 430072, People's Republic of China\\
$^{66}$ Xinyang Normal University, Xinyang 464000, People's Republic of China\\
$^{67}$ Zhejiang University, Hangzhou 310027, People's Republic of China\\
$^{68}$ Zhengzhou University, Zhengzhou 450001, People's Republic of China\\
\vspace{0.2cm}
$^{a}$ Also at Bogazici University, 34342 Istanbul, Turkey\\
$^{b}$ Also at the Moscow Institute of Physics and Technology, Moscow 141700, Russia\\
$^{c}$ Also at the Novosibirsk State University, Novosibirsk, 630090, Russia\\
$^{d}$ Also at the NRC "Kurchatov Institute", PNPI, 188300, Gatchina, Russia\\
$^{e}$ Also at Istanbul Arel University, 34295 Istanbul, Turkey\\
$^{f}$ Also at Goethe University Frankfurt, 60323 Frankfurt am Main, Germany\\
$^{g}$ Also at Key Laboratory for Particle Physics, Astrophysics and Cosmology, Ministry of Education; Shanghai Key Laboratory for Particle Physics and Cosmology; Institute of Nuclear and Particle Physics, Shanghai 200240, People's Republic of China\\
$^{h}$ Also at Key Laboratory of Nuclear Physics and Ion-beam Application (MOE) and Institute of Modern Physics, Fudan University, Shanghai 200443, People's Republic of China\\
$^{i}$ Also at Harvard University, Department of Physics, Cambridge, MA, 02138, USA\\
$^{j}$ Currently at: Institute of Physics and Technology, Peace Ave.54B, Ulaanbaatar 13330, Mongolia\\
$^{k}$ Also at State Key Laboratory of Nuclear Physics and Technology, Peking University, Beijing 100871, People's Republic of China\\
$^{l}$ School of Physics and Electronics, Hunan University, Changsha 410082, China\\
}\end{center}
\vspace{0.4cm}
\end{small}
}
\noaffiliation{}

